Bellman Residual Orthogonalization for Offline Reinforcement Learning

We propose and analyze a reinforcement learning principle that approximates the Bellman equations by enforcing their validity only along an user-defined space of test functions. Focusing on applications to model-free offline RL with function approximation, we exploit this principle to derive confidence intervals for off-policy evaluation, as well as to optimize over policies within a prescribed policy class. We prove an oracle inequality on our policy optimization procedure in terms of a trade-off between the value and uncertainty of an arbitrary comparator policy. Different choices of test function spaces allow us to tackle different problems within a common framework. We characterize the loss of efficiency in moving from on-policy to off-policy data using our procedures, and establish connections to concentrability coefficients studied in past work. We examine in depth the implementation of our methods with linear function approximation, and provide theoretical guarantees with polynomial-time implementations even when Bellman closure does not hold.

==> 3p1p2-Overview.tex <==
\subsection{Overview of paper}

In this paper, we show how the principle of Bellman residual
orthogonalization can be used to develop useful methods for off-policy
evaluation and optimization.  In \cref{sec:Algorithms}, we propose a
data-based method for approximately solving the weak Bellman
equations~\eqref{eqn:WeakFormulation} induced by a given test class,
and show how it can be used to compute a high probability confidence
interval---that is, upper and lower bounds---on the value function of
any policy.  In turn, by maximizing the lower envelope of these value
estimates, we can perform approximate policy optimization by solving a
max-min problem.  We then analyze the behavior of this procedure,
first by providing a deterministic result (\cref{prop:Deterministic}) that
controls the width of the confidence intervals, and then a
guarantee on the max-min procedure for policy optimization.  Using
this result as guidance, we then prove that under a fairly general
model for data generation, our estimators yield the desired behavior
with high probability.  This result, stated
as~\cref{thm:NewPolicyEvaluation}, involves the metric entropies of
the three function classes---the test space, the $Q$-function space,
and the policy class.  In Corollaries~\ref{cor:poly}
and~\ref{cor:alpha}, we instantiate this general result for function
classes with various types of metric entropy.


Section~\ref{sec:Applications} is motivated by the question: what is
the ``cost'' of off-policy data relative to the more benign on-policy
setting?  In order to provide some insight, we define an {\goodname}
$\ConcSimple$ that measures the inflation in our bounds
incurred by moving from on-policy to off-policy data.  We show that
this coefficient can be upper bounded in terms of quantities
introduced in past work on the off-policy setting, including the
likelihood ratio along with various types of concentrability
coefficients.  We also discuss the choice of test function class, and
how it interacts with the {\goodname}.

In \cref{sec:Linear}, we specialize to the linear setting, and propose
a computationally tractable manner in which to implement the max-min
problem that underlies our policy optimization procedure.  We work
with the class of soft-max policies, and show that a variant of a
mirror descent procedure, when analyzed in an adversarial and online
setting, can be used to solve the max-min problem in a computationally
efficient manner.  The main result of this section
(\cref{thm:LinearApproximation}) provides an explicit upper bound on
the performance of the policy computed by our algorithm.



Apart from these specific contributions, the applicability of this
principle may extend beyond the offline setting considered here.  It
allows our procedures to operate under a ``weak'' realizability
assumption, to derive new concentrability coefficients as well as to
recover existing ones thanks to the flexibility afforded by the test
space.


==> 3p2p1-arxiv.tex <==
We begin by introducing background, and setting up the problem to be
studied.

\subsection{Preliminaries}

In this paper, we focus on infinite-horizon discounted Markov decision
processes~\cite{puterman1994markov,bertsekas1996neuro,sutton2018reinforcement}
specified by a discount factor $\discount \in [0,1)$, a state space
  $\StateSpace$, and an action set $\ActionSpace$.  For each
  state-action pair $\psa$, there is a reward distribution
  $\RewardLaw\psa$ supported on the interval $[0,1]$ with mean
  $\reward\psa$, along with a probability transition function
  $\TransitionLaw(\cdot \mid \state, \action)$.

\paragraph{Value functions and Bellman evaluation:}  
A (stationary) stochastic policy $\policy$ is a mapping from the state
space to a distribution over the action space---that is, a mapping
$\state \mapsto \policy(\cdot \mid \state)$.  For a given policy, its
$Q$-function or action-value function is the discounted sum of future
rewards based on starting from the pair $\psa$, and then following the
policy $\policy$ in all future time steps.  More precisely, it is
given by
\begin{subequations}
\begin{align}
\Qfnc^{\pi}\psa = \reward\psa + \sum_{\hstep = 0}^{\infty}
\discount^{\hstep} \Exp \Big[ \reward_{\hstep}({\SState}_\hstep,
  {\AAction}_\hstep) \mid (\SState_0, \AAction_0) = \psa \Big],
\end{align}
where the expectation is taken over trajectories with
\begin{align}
\label{EqnTrajectory}
\AAction_{\hstep} \sim \pol(\cdot \mid \SState_\hstep), \quad
\mbox{and} \quad \SState_{\hstep+1} \sim \TransitionLaw(\cdot \mid
\SState_\hstep, \AAction_\hstep) \quad \mbox{for $\hstep = 1, 2,
  \ldots,$.}
\end{align}
\end{subequations}
We also make use of the convenient shorthand $\Qpi{\policy}(\state,
\policy) \defeq \Expecti{\Qpi{\policy}(\state, \AAction)}{\AAction
  \sim \policy(\cdot \mid \state)}$.  The state-action value function
$\Qpi{\policy}$ is known to be the unique fixed point of the
\emph{Bellman evaluation operator}
\begin{subequations}
\begin{align}
(\BellmanEvaluation{\policy}\Qfnc)\psa = \reward\psa +
  \Expecti{\Qfnc(\SState^+ ,\policy)} {\SState^+ \sim
    \TransitionLaw(\cdot \mid \state, \action)},
\end{align}
Moreover, it is known to be related to the state-value function via
the relation
\begin{align}
\Vpi{\policy}(\state) = \Qpi{\policy}(\state,\policy).
\end{align}
\end{subequations}
In our analysis, we assume that policies have action-value functions
that satisfy the uniform bound $\sup_{\psa} \abs{\Qpi{\policy}\psa}
\leq 1$.  It should be noted that this constraint (modulo a suitable
rescaling) allows for a broader class of models than one in which the
rewards are bounded in $[0,1]$; see the
papers~\cite{jiang2018open,zanette2019tighter} for details.


We are also interested in approximating optimal policies.  Under some
regularity conditions~\cite{puterman1994markov,shreve1978alternative},
there always exists an optimal policy $\pistar$ whose value and
action-value functions are defined as $\Vstar(\state) =
V^{\pistar}(\state) = \sup_{\policy} \Vpi{\policy}(\state)$ and
$\Qstar\psa = \Qfnc^{\pistar}\psa = \sup_{\policy}
\Qfnc^{\policy}\psa$.

\paragraph{Discounted occupancy measures:}
Throughout the paper, we assume that the starting state $\SState_0$ is
drawn according to some initial distribution $\startdistribution$.  We
study the scalarized value given by
\begin{align}
  \Vpi{\policy} & \defeq \Exp_{\SState_0 \sim
    \startdistribution}[\Vpi{\policy}(\SState_0)],
\end{align}
corresponding to value function averaged over the random choice
of starting state.

Our results and analysis make extensive use of the \emph{discounted
occupancy measure} associated with a policy $\policy$, defined as
follows.  Suppose that we generate trajectories by drawing the initial
state $\SState_0 \sim \startdistribution$ and action $\AAction_0 \sim
\policy(\cdot \mid \SState_0)$, and then following the standard
trajectory model~\eqref{EqnTrajectory} at all subsequent time steps.
For each time step $\hstep = 0, 1, 2, \ldots$, let $\Prob_\hstep$
denote the marginal distribution over state-action pairs at time
$\hstep$ induced by this data-generation procedure.  Then the
\emph{discounted occupancy measure} for policy $\policy$ is given by
\begin{align}
\DistributionOfPolicy{\policy}\psa & \defeq (1 - \discount )
\sum_{\hstep=0}^\infty \discount^\hstep \Pro_\hstep\Big[
  (\SState_\hstep,\AAction_\hstep) = \psa \Big].
\end{align}
Among other reasons, this measure is convenient in that it leads
to compact representations for value functions.  In particular,
the definition ensures that
\begin{align}
\Expecti{[\reward(\SState, \AAction)]}{(\SState, \AAction) \sim
  \DistributionOfPolicy{\policy}} = (1-\discount) \Vpi{\policy}.
\end{align}
More generally, we adopt the shorthand notation $\Exp_\policy$ for
expectations over $\DistributionOfPolicy{\policy}$.  For any functions
$f, g: \StateSpace \times \ActionSpace \rightarrow \R$, we make
frequent use of the shorthands
\begin{align*}
\Exp_\policy[f] \defeq \Exp_{(\SState, \AAction) \sim
  \DistributionOfPolicy{\policy}}[f(\SState, \AAction)], \quad
\mbox{and} \quad \inprod{f}{g}_\policy \defeq \Exp_{(\SState,
  \AAction) \sim \DistributionOfPolicy{\policy}} \big[f(\SState,
  \AAction) \, g(\SState, \AAction) \big].
\end{align*}
Note moreover that we have $\inprod{\1}{f}_\policy = \Exp_\policy[f]$
where $\1$ denotes the identity function.

\paragraph{TD and Bellman errors:} For a given $\Qfnc$-function and
policy $\policy$, let us define the \emph{temporal difference error}
(or TD error) associated with the sample $\sarsizNp{} = \sars{}$ and
the \emph{Bellman error} at $\psa$
\begin{subequations}
\begin{align}
(\TDError{\Qfnc}{\policy}{})\sarsiz{} \defeq \Qfnc\psa - \reward -
  \gamma \Qfnc(\successorstate,\policy), \qquad
  (\BellmanError{\Qfnc}{\policy}{})\psa \defeq \Qfnc\psa - \reward\psa
  - \gamma
  \E_{\successorstate\sim\TransitionLaw\psa}\Qfnc(\successorstate,\policy).
\end{align}
The TD error is a random variable function of $\sarsizNp{}$, while the
Bellman error is its conditional expectation with respect to the
immediate reward and successor state at $\psa$.
Many of our bounds involve the quantity
\begin{align}
\Expecti{\BellmanError{\Qfnc}{\policy}{}}{\policy} \defeq
\Expecti{\big[\BellmanError{\Qfnc}{\policy}{} \PSA \big]} {\PSA \sim
  \DistributionOfPolicy{\policy}}.
\end{align}
\end{subequations}

\subsection{Function Spaces and Weak Representation}

Our methods involve three different types of function spaces,
corresponding to policies, action-value functions, and test
functions. Recall that a stationary stochastic policy is a mapping from
each state $\state$ to a probability distribution $\policy(\cdot \mid
\state)$ over the action space.  An action-value function is a mapping
$\psa \mapsto \Qfnc \psa \in [0,1]$.  A test function
$\TestFunction{}$ is a mapping $\psai \mapsto \TestFunction{}\psai$,
where $\identifier$ is an optional identifier containing side
information.  Without loss of generality (rescaling as necessary), we
may assume that \mbox{$\sup_{\psai}\abs{\TestFunction{}\psai} \leq
  1$.} \\

\noindent Our methodology involves the following three function
classes:
\begin{itemize}
\item a \emph{policy class} $\PolicyClass$ that contains all policies
  $\policy$ of interest (for evaluation or optimization);
\item for each $\policy$, the \emph{predictor class}
  $\Qclass{\policy}$ of action-value functions $Q$ that we permit; and
\item for each $\policy$, the \emph{test function class}
  $\TestFunctionClass{\policy}$ that we use to enforce the Bellman
  residual constraints.
\end{itemize}
\noindent The union over all the predictor spaces is denoted by
$\Qclass{} = \cup_{\policy \in \PolicyClass}\Qclass{\policy}$, and
similarly, we let \mbox{$\TestFunctionClass{} = \cup_{\policy \in
    \PolicyClass} \TestFunctionClass{\policy}$} denote the union over
all test spaces for the policies. \\
 
\noindent Throughout the paper, we assume \emph{weak realizability}
with respect to the policies in $\PolicyClass$.
\begin{assumption}[Weak Realizability]
\label{asm:WeakRealizability}
For a given policy $\policy$, the predictor class $\Qclass{\policy}$
is weakly realizable with respect to the test space
$\TestFunctionClass{\policy}$ and the measure
$\DatasetDistributionStateActions$ if there exists a predictor
$\QpiWeak{\policy} \in \Qclass{\policy}$ such that
\begin{align}
\label{EqnWeakRealizable}  
\innerprodweighted{\TestFunction{}}
                  {\BellmanError{\QpiWeak{\policy}}{\policy}{}}
                  {\DatasetDistributionStateActions} = 0 \; \text{for
                    all } \TestFunction{} \in
                  \TestFunctionClass{\policy} \qquad \text{and} \qquad
                  \innerprodweighted{\1}{\BellmanError{\QpiWeak{\policy}}{\policy}{}}{\policy}
                  = 0.
	\end{align}
\end{assumption}
The first condition requires the predictor to satisfy the weak Bellman
equations \eqref{eqn:WeakFormulation}.  The second condition amounts
to requiring that the predictor returns the value of $\policy$ at the
start distribution: using \cref{lem:Simulation} stated in the sequel,
we have
\begin{align}
\Expecti{\QpiWeak{\policy}(\MyState ,\policy)}{\MyState \sim
  \startdistribution} - \Vpi{\policy} =
\Expecti{[\QpiWeak{\policy}-\Qpi{\policy}](\MyState
  ,\policy)}{\MyState \sim \startdistribution} = \horizon
\Expecti{\BellmanError{\QpiWeak{\policy}}{\policy}{}}{\policy} =
\horizon
\innerprodweighted{\1}{\BellmanError{\QpiWeak{\policy}}{\policy}{}}{\policy}
= 0.
\end{align}
This weak notion should be contrasted with \emph{strong
realizability}, which means that the true value function
$\Qpi{\policy}$ belongs to $\Qclass{\policy}$, meaning that there is a
function in $\Qclass{\policy}$ that satisfies the Bellman equation in
all state-action pairs.  Weak realizability is a much milder
requirement than strong realizability, because the weak solution
$\QpiWeak{\policy}$ only needs to satisfy the Bellman equations in an
average sense for functions in $\TestFunctionClass{\policy}$.

For future reference, we also state a notion of weak closure.  (To be
clear, no form of closure will be assumed in our results unless
otherwise stated.)
\begin{definition}[Weak Bellman Closure]
The Bellman operator $\BellmanEvaluation{\policy}$ is \emph{weakly
closed} with respect to the triple $\big( \Qclass{\policy},
\TestFunctionClass{\policy}, \DatasetDistributionStateActions \big)$
if for any $\Qfnc \in \Qclass{\policy}$, there exists a predictor
$\QpiProj{\policy}{\Qfnc} \in \Qclass{\policy}$ such that
\begin{align}  
\innerprodweighted{\TestFunction{}}{\QpiProj{\policy}{\Qfnc}}{\DatasetDistributionStateActions}
= \innerprodweighted{\TestFunction{}}
{\BellmanEvaluation{\policy}(\Qfnc)}
{\DatasetDistributionStateActions}.
\end{align}
\end{definition}
\noindent As reflected in our choice of terminology, this requirement
is less restrictive than \emph{strong Bellman closure}, which requires
that
\begin{align}
\BellmanEvaluation{\policy}(\Qfnc) \in \Qclass{\policy} \qquad
\mbox{for all $\Qfnc \in \Qclass{\policy}$.}
\end{align}



==> 3p3-arxiv.tex <==

\section{Policy Estimates via the Weak Bellman Equations}
\label{sec:Algorithms}

In this section, we describe procedures for both off-policy evaluation
and optimization that are based on the weak Bellman equations.  Our
method for policy optimization exploits the fact that any predictor
$\Qfnc$ that approximately solves the weak Bellman equations can be
used to make off-policy predictions for policy improvement.
Therefore, our first step is to approximately solve the weak
formulation~\eqref{eqn:WeakFormulation}.  In practice, the Bellman
operator is not explicitly known, but we can form an empirical
approximation using a given dataset $\Dataset$.  In this section, we
introduce a general method for doing so, and then use it to derive
confidence intervals for off-policy prediction and then for policy
optimization using pessimism.

\subsection{Weighted temporal differences and empirical constraints}  


Given a dataset $\Dataset = \{(\state_i, \action_i, \reward_i,
\successorstate_i) \}_{i=1}^\numobs$, we can approximate the Bellman
errors in the weak Bellman equations \eqref{eqn:WeakFormulation} by a
linear combination of the temporal difference errors:
\begin{align}
\label{eqn:WeightedTemporaResidual}
\int \TestFunction{}\psa \underbrace{[\Qfnc\psa -
    (\BellmanEvaluation{\policy} \Qfnc)\psa]}_{=
  \BellmanError{\Qfnc}{\policy}{}\psa }
d\DatasetDistributionStateActions \approx \frac{1}{\nSamples}
\sum_{i=1}^\numobs \TestFunction{}\psaindex \underbrace{ [\Qfnc\psaindex -
    \reward_i - \discount \Qfnc(\successorstate_i,\policy) ]}_{=
  \TDError{\Qfnc}{\policy}{}\sarsi{i} }.
\end{align}
Note that the approximation~\eqref{eqn:WeightedTemporaResidual}
corresponds to a weighted linear combination of temporal differences,
where the weights are determined by the test functions.  So as to
streamline our notation, let us define the empirical inner product
\begin{align*}
  \inprod{\TestFunction{}}{ \TDError{\Qfnc}{\policy}{}}_\numobs &
  \defeq \frac{1}{\nSamples} \sum_{i=1}^\numobs
  \TestFunction{}\psaindex [\Qfnc\psaindex - \reward_i - \discount
    \Qfnc(\successorstate_i,\policy) ]
\end{align*}
so that an equivalent form of
equation~\eqref{eqn:WeightedTemporaResidual} is
$\innerprodweighted{\TestFunction{}}{\BellmanError{\Qfnc}{\policy}{}}{\mudist}
\approx
\innerprodweighted{\TestFunction{}}{\TDError{\Qfnc}{\policy}{}}{\mudist}$. This
simple plug-in approximation works because the TD errors are noisy
estimates of the Bellman errors, and hence the linear combinations of
the TD errors are linear combinations of the Bellman errors plus some
decaying noise due to averaging in the linear combinations.  The
double sampling issue---a curse of methods that attempt to minimize
the squared Bellman error---is avoided because only linear
combinations of the noise are performed as opposed to operations that
``square the noise'' and introduce bias.

We now specify a set of approximate solutions to the weak Bellman
equations using these weighted temporal differences.  Since the
empirical approximation \eqref{eqn:WeightedTemporaResidual} introduces
sampling errors, we instead require only inequalities (as opposed to
equality constraints) in the weak Bellman equation for each test
function.  Given a class of test functions
$\TestFunctionClass{\policy}$, a radius parameter $\Rad \geq 0$ and
regularization parameter $\regpar \geq 0$, we define the set
\begin{align}
\label{eqn:EmpiricalBellmanGalerkinEquations}
\SuperEmpiricalFeasible \defeq \left \{ \Qfnc \in \Qclass{\policy}
\quad \text{such that} \quad
\sup_{\TestFunction{}\in\TestFunctionClass{\policy}} \frac{
  \abs{\innerprodweighted{\TestFunction{}}{\TDError{\Qfnc}{\pi}{}}{\nSamples}}
} { \TestNormaRegularizerEmp{} } \leq \sqrt{\frac{\Rad}{\nSamples}}
\quad \mbox{for all $\testfunc \in \TestFunctionClass{}$}\right \}.
\end{align}
When the choices of $(\Rad, \regpar)$ are clear from the context, we
adopt the shorthand $\EmpiricalFeasibleSet{\policy}(
\TestFunctionClass{\policy})$, or $\EmpiricalFeasibleSet{\policy}$
when the function class $\TestFunctionClass{\policy}$ is also clear.

The division by $\TestNormaRegularizerEmp{}$ in each constraint that
define membership in the set ensures that the constraint is
self-normalizing.  The regularization parameter $\regpar$ serves to
avoid blow-up due to functions whose squared empirical norm
$\EmpNorm{f}^2 \defeq \frac{1}{\numobs} \sum_{i=1}^\numobs
f^2(\state_i, \action_i)$ is very close to zero.  On the other hand,
the radius parameter $\Rad$ controls the tightness of the constraints
that define membership in $\EmpiricalFeasibleSet{\policy}$.  As
detailed in the sequel, it should be chosen to depend on the
complexity of the three underlying function spaces (test, policy, and
$Q$-function).  In our concrete result to be stated in the sequel, we
do so based on certain metric entropies of these function classes.
Finally, note that the right-hand side of the constraint decays as
$1/\sqrt{\nSamples}$, so that the weak Bellman constraints are
enforced more tightly as the sample size increases.

We now describe how any set of the
form~\eqref{eqn:EmpiricalBellmanGalerkinEquations} leads to procedures
for policy evaluation and optimization.

\paragraph{Confidence bounds for policy evaluation:}
First, for any fixed policy $\policy$, we can use the feasibility
set~\eqref{eqn:EmpiricalBellmanGalerkinEquations} to compute the lower
and upper estimtes
\begin{align}
\label{eqn:ConfidenceIntervalEmpirical}
\VminEmp{\policy} \defeq \min_{\Qfnc \in \SuperEmpiricalFeasible}
\Expecti{\big[\Qfnc(\MyState ,\policy)\big]}{\MyState \sim
  \startdistribution}, \qquad \text{and} \quad \VmaxEmp{\policy}
\defeq \max_{\Qfnc \in \SuperEmpiricalFeasible}
\Expecti{\big[\Qfnc(\MyState ,\policy)\big]}{\MyState \sim
  \startdistribution},
\end{align} 
corresponding to estimates of the minimum and maximum value that the
policy $\policy$ can take at the initial distribution.\footnote{Note
that strictly speaking, these estimates depend on the triple $(\Rad,
\regpar, \TestFunctionClass{\policy})$, but we omit this dependence so
as not to clutter the notation.}  In the sequel, we give conditions
under which these upper/lower estimates actually provide bounds on the
true value function, so that they can define valid confidence
intervals.


\paragraph{Max-min estimate for policy optmization:}

We have defined a procedure for computing the $\policy \mapsto
\VminEmp{\policy}$, which provides a lower estimate for the value of
any policy.  This family of lower estimates can be used to perform
policy optimization over the class $\PolicyClass$, in particular by
solving the \emph{max-min} problem
\begin{align}
\label{eqn:MaxMinEmpirical}
  \max_{\pInP} \Big [\min_{\Qfnc \in \EmpiricalFeasibleSet{\policy}}
    \Expecti{\Qfnc(\MyState ,\policy)}{\MyState \sim
      \startdistribution} \Big], \qquad \text{or equivalently} \qquad
  \max_{\pInP}\VminEmp{\policy}.
\end{align}
In the sequel, we prove an oracle inequality for this max-min
estimator, in particular one that involves, for an arbitrary
comparator policy $\pi$, a trade-off between its value and a measure
of its evaluation uncertainty.


\subsection{Form of guarantees}

Let us now specify and discuss the types of guarantees that we
establish for our estimators~\eqref{eqn:ConfidenceIntervalEmpirical}
and~\eqref{eqn:MaxMinEmpirical}.  All of our theoretical guarantees
involve a $\mudist$-based counterpart
$\PopulationFeasibleSet{\policy}$ of the data-dependent set
$\EmpiricalFeasibleSet{\policy}$.  It is obtained via the following
changes:
%
\bcar
\item replacing the empirical inner products and norms induced by the
  dataset $\Dataset$ by their population versions associated with
  $\mu$;
\item replacing the temporal difference error
  $\TDError{\Qfnc}{\policy}{}$ with the Bellman error
  $\BellmanError{\Qfnc}{\policy}{}$;
\item suitably enlarging the radius parameter. (For concreteness, we
  replace $\Rad$ by $4 \Rad$.)  \ecar

\vspace*{0.05in}

  
\noindent More precisely, we define the set
\begin{align}
\label{eqn:ApproximateBellmanGalerkingEquations}
\SuperPopulationFeasible \defeq \Big\{ \Qfnc \in \Qclass{\policy}
\quad \text{such that} \quad \frac{
  \abs{\innerprodweighted{\TestFunction{}}{\BellmanError{\Qfnc}{\pi}{}}{\DatasetDistributionStateActions}}
} { \TestNormaRegularizerPop{} } \leq \sqrt{\frac{4 \Rad}{\nSamples}}
\qquad \mbox{for all $\testfunc \in \TestFunctionClass{}$} \Big\},
\end{align}
where $\inprod{f}{g}_\DatasetDistributionStateActions \defeq \int f
\psa g \psa d \mu$ is the inner product induced by a
distribution\footnote{See Section~\ref{SecDataGen} for a precise
definition of the relevant $\mu$ for a fairly general sampling model.}
$\mu$ over $\psa$.  As before, we use the shorthand notation
$\PopulationFeasibleSet{\policy}$ when the underlying arguments are
clear from context.  Moreover, in the sequel, we generally ignore the
constant $4$ in the
definition~\eqref{eqn:ApproximateBellmanGalerkingEquations} by
assuming that $\Rad$ is rescaled appropriately---e.g., that we use a
factor of $\tfrac{1}{4}$ in defining the empirical set.


It should be noted that in contrast to the set
$\EmpiricalFeasibleSet{\policy}$, the set
$\PopulationFeasibleSet{\policy}$ is defined in terms of the
distribution $\DatasetDistributionStateActions$ and the input space
$\InputFunctionalSpace$.  It relaxes the orthogonality constraints in
the weak Bellman formulation~\eqref{eqn:WeakFormulation} to a form of
\emph{approximate orthogonality}, as controlled by the pair $(\Rad,
\regpar)$ along with the sample size $\numobs$.  Given this
definition, we are now ready to describe the types of guarantees
proved in this paper:

\paragraph{Confidence intervals for policy evaluation:}
For any fixed policy, our main results provide sufficient conditions
for the upper-lower estimates~\eqref{eqn:ConfidenceIntervalEmpirical}
to satisfy the following two properties:
\begin{subequations}
\label{EqnPolEval}  
\begin{align}
\label{EqnCoverage}
\mbox{\underline{Coverage guarantee:}} & \qquad \big[
  \VminEmp{\policy}, \VmaxEmp{\policy} \big] \ni \Vpi{\policy}. \\
%
  \label{EqnWidthBound}
\mbox{\underline{Width bound:}} & \qquad \max \Big \{
|\VminEmp{\policy} - \Vpi{\policy} |, \; |\VmaxEmp{\policy} -
\Vpi{\policy} | \Big \} \leq \horizon \max_{\Qfnc \in
  \PopulationFeasibleSet{\policy}(\TestFunctionClass{\policy})}
|\PolComplex|.
  \end{align}
\end{subequations}
When both of these guarantees hold with probability $1 - \delta$, then
condition~\eqref{EqnCoverage} amounts to asserting that $\big[
  \VminEmp{\policy}, \VmaxEmp{\policy} \big]$ is a confidence interval
with coverage $1 - \delta$, whereas the bound~\eqref{EqnWidthBound}
provides control on the width of this confidence interval.

\paragraph{Oracle inequality for policy optimization:}
Turning to the more challenging setting of policy optimization, our
main results give sufficient conditions for any policy $\piemp$
obtained from the max-min criterion~\eqref{eqn:MaxMinEmpirical} to
satisfy the family of lower bounds
\begin{align}
\label{EqnOracle}
\mbox{\underline{Oracle inequality:}} \qquad \Vpi{\piemp} \geq
\max_{\policy \in \PolicyClass} \Biggr \{
\underbrace{
\vphantom{
\frac{1}{1 - \discount} \max_{\Qfnc \in
    \PopulationFeasibleSet{\policy}(\TestFunctionClass{})}
  |\PolComplex|
  }
\Vpi{\policy}}_{\mbox{\tiny{Value}}} -
\underbrace{\frac{1}{1 - \discount} \max_{\Qfnc \in
    \PopulationFeasibleSet{\policy}(\TestFunctionClass{})}
  |\PolComplex|}_{\mbox{\tiny{Evaluation uncertainty}}} \Biggr \}.
  \end{align}
To explain the terminology, equation~\eqref{EqnOracle} provides a
family of lower bounds, one for each choice of the policy $\policy$.
Each lower bound involves a trade-off between the value
$\Vpi{\policy}$ of the policy and its evaluation uncertainty.  While
no practical procedure has direct access to these values and
evaluation uncertainties, inequality~\eqref{EqnOracle} shows that the
max-min estimator returns a value that is at least as good as the
optimal trade-off obtained by an oracle that has access to these
values, and can search over all policies.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{A deterministic guarantee}

We begin our analysis stating a deterministic set of sufficient
conditions for our estimators to satisfy the
guarantees~\eqref{EqnPolEval} and~\eqref{EqnOracle}.  This formulation
is useful, because it reveals the structural conditions that underlie
success of our estimators, and in particular the connection to weak
realizability.  In Section~\ref{SecHighProb}, we exploit this
deterministic result to show that, under a fairly general sampling
model, our estimators enjoy these guarantees with high probability.


In the previous section, we introduced the population level set
$\PopulationFeasibleSet{\policy}$ that arises in the statement of our
guarantees.  Also central in our analysis is the infinite data limit
of this set.  More specifically, for any fixed $(\Rad, \regpar)$, if
we take the limit $\nSamples \rightarrow \infty$, then
$\PopulationFeasibleSet{\policy}$ reduces to the set of all solutions
to the weak formulation~\eqref{eqn:WeakFormulation}---that is
\begin{align}
\PopulationFeasibleSetInfty{\policy}(\TestFunctionClass{\policy}) = \{
\Qfnc \in \Qclass{\policy} \mid
\innerprodweighted{\TestFunction{}}{\BellmanError{\Qfnc}{\pi}{}}
                  {\DatasetDistributionStateActions} = 0 \quad
                  \mbox{for all $\TestFunction{} \in
                    \TestFunctionClass{\policy}$} \}.
\end{align}
As before, we omit the dependence on the test function class
$\TestFunctionClass{\policy}$ when it is clear from context. By
construction, we have the inclusion
$\PopulationFeasibleSetInfty{\policy}(\TestFunctionClass{\policy})
\subseteq \SuperPopulationFeasible$ for any non-negative pair $(\Rad,
\regpar)$.

\vspace*{0.05in}


Our first set of guarantees hold when the random set
$\EmpiricalFeasibleSet{\policy}$ satisfies the \emph{sandwich
relation}
\begin{align}
\label{EqnSandwich}  
\PopulationFeasibleSetInfty{\policy}(\TestFunctionClass{\policy})
\subseteq \EmpiricalFeasibleSet{\policy}(\Rad, \regpar;
\TestFunctionClass{\policy}) \subseteq
\PopulationFeasibleSet{\policy}(4 \Rad, \regpar;
\TestFunctionClass{\policy})
\end{align}
To provide intuition as to why this sandwich condition is natural,
observe that it has two important implications:
\begin{enumerate}
\item[(a)] Recalling the definition of weak
  realizability~\eqref{EqnWeakRealizable}, the weak solution
  $\QpiWeak{\policy}$ belongs to the empirical constraint set
  $\EmpiricalFeasibleSet{\policy}$ for any choice of test function
  space.  This important property follows because $\QpiWeak{\policy}$
  must satisfy the constraints~\eqref{eqn:WeakFormulation}, and thus
  it belongs to $\PopulationFeasibleSetInfty{\policy} \subseteq
  \EmpiricalFeasibleSet{\policy}$.
%
\item[(b)] All solutions in $\EmpiricalFeasibleSet{\policy}$ also
  belong to $\PopulationFeasibleSet{\policy}$, which means they
  approximately satisfy the weak Bellman equations in a way quantified
  by $\PopulationFeasibleSet{\policy}$.
\end{enumerate}
By leveraging these facts in the appropriate way, we can establish
the following guarantee: \\


\begin{proposition}
\label{prop:Deterministic}
The following two statements hold. 
\begin{enumerate}
\item[(a)] \underline{Policy evaluation:} If the set
  $\EmpiricalFeasibleSet{\policy}$ satisfies the sandwich
  relation~\eqref{EqnSandwich}, then the estimates
  $(\VminEmp{\policy}, \VmaxEmp{\policy})$ satisfy the width
  bound~\eqref{EqnWidthBound}.  If, in addition, weak Bellman
  realizability for $\policy$ is assumed, then the
  coverage~\eqref{EqnCoverage} condition holds.
%
\item[(b)] \underline{Policy optimization:} If the sandwich
  relation~\eqref{EqnSandwich} and weak Bellman realizability hold for
  all $\policy \in \PolicyClass$, then any
  max-min~\eqref{eqn:MaxMinEmpirical} optimal policy $\piemp$
  satisfies the oracle inequality~\eqref{EqnOracle}.
\end{enumerate}
\end{proposition}
\noindent See Section~\ref{SecProofPropDeterministic} for the proof of
this claim. \\

In summary, \Cref{prop:Deterministic} ensures that when weak
realizability is in force, then the sandwich
relation~\eqref{EqnSandwich} is a sufficient condition for both the
policy evaluation~\eqref{EqnPolEval} and
optimization~\eqref{EqnOracle} guarantees to hold.  Accordingly, the
next phase of our analysis focuses on deriving sufficient conditions
for the sandwich relation to hold with high probabability.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Some high-probability guarantees}
\label{SecHighProb}

As stated, \Cref{prop:Deterministic} is a ``meta-result'', in that it
applies to any choice of set $\EmpiricalFeasibleSet{\policy} \equiv
\SuperEmpiricalFeasible$ for which the sandwich
relation~\eqref{EqnSandwich} holds.  In order to obtain a more
concrete guarantee, we need to impose assumptions on the way in which
the dataset was generated, and concrete choices of $(\Rad, \regpar)$
that suffice to ensure that the associated sandwich
relation~\eqref{EqnSandwich} holds with high probability.  These tasks
are the focus of this section.


\subsubsection{A model for data generation}
\label{SecDataGen}
Let us begin by describing a fairly general model for data-generation.
Any sample takes the form $\sarsizNp{} \defeq \sarsi{}$, where the
five components are defined as follows:
\vspace{0.04in}
\bcar
\item the pair $(\state, \action)$ index the current state and action.
\item the random variable $\reward$ is a noisy observation of the mean
  reward.
\item the random state $\successorstate$ is the next-state sample,
  drawn according to the transition $\TransitionLaw\psa$.
\item the variable $\identifier$ is an optional identifier.
  %
  \ecar 

\vspace{0.04in}  
\noindent As one example of the use of an identifier variable, if
samples might be generated by one of two possible policies---say
$\policy_1$ and $\policy_2$---the identifier can take values in the
set $\{1, 2 \}$ to indicate which policy was used for a particular
sample. \\

Overall, we observe a dataset $\Dataset = \{\sarsizNp{i}
\}_{i=1}^\numobs$ of $\numobs$ such quintuples.  In the simplest of
possible settings, each triple $\psai$ is drawn i.i.d.  from some
fixed distribution $\DatasetDistributionStateActions$, and the noisy
reward $\reward_i$ is an unbiased estimate of the mean reward function
$\Reward(\state_i, \action_i)$.  In this case, our dataset consists of
$\numobs$ i.i.d.  quintuples.  More generally, we would like to
accommodate richer sampling models in which the sample $z_i =
(\state_i, \action_i, \identifier_i, \reward_i, \successorstate_i)$ at
a given time $i$ is allowed to depend on past samples.  In order to
specify such dependence in a precise way, define the nested sequence
of sigma-fields
\begin{align}
\Filtration_1 = \emptyset, \quad \mbox{and} \quad \Filtration_i \defeq
\sigma \Big(\{\sarsizNp{j}\}_{j=1}^{i-1} \Big) \qquad \mbox{for $i =
  2, \ldots, \numobs$.}
\end{align}
In terms of this filtration, we make the following definition:

\begin{assumption}[Adapted dataset]
  \label{asm:Dataset}
  An adapted dataset is a collection $\Dataset = \{
  \sarsizNp{\iSample} \}_{i=1}^\numobs$ such that for each $i = 1,
  \ldots, \numobs$:
%
\bcar
\item There is a conditional distribution
  $\DatasetDistributionStateActions_i$ such that $(\state_i,
  \action_i, \identifier_i) \sim \DatasetDistributionStateActions_i
  (\cdot \mid \Filtration_i)$.
\item Conditioned on
  $(\state_\iSample,\action_\iSample,\identifier_\iSample )$, we
  observe a noisy reward $\reward_\iSample =
  \reward(\state_\iSample,\action_\iSample) + \eta_i$ with $\E[\eta_i
    \mid \Filtration_{\iSample} ] = 0$, and $|\reward_i| \leq 1$.
  %
\item Conditioned on
  $(\state_\iSample,\action_\iSample,\identifier_\iSample )$, 
  the next state $\successorstate_\iSample$ is generated
  according to
  $\TransitionLaw(\state_\iSample,\action_\iSample)$.
%
\ecar
\end{assumption}


Under this assumption, we can define the (possibly) random reference
measure
\begin{align}
\DatasetDistributionStateActions(\state, \action, \identifier) &
\defeq \frac{1}{\numobs} \sum_{i=1}^\numobs
\DatasetDistributionStateActions_i \big(\state, \action, \identifier
\mid \Filtration_i \big).
\end{align}
In words, it corresponds to the distribution induced by first drawing
a time index $i \in \{1, \ldots, \numobs \}$ uniformly at random, and
then sampling a triple $\psai$ from the conditional distribution
$\DatasetDistributionStateActions_i \big(\cdot \mid \Filtration_i
\big)$.





\subsubsection{A general guarantee}
\newcommand{\Mfun}{\ensuremath{\phi}}
\label{SecGeneral}


Recall that there are three function classes that underlie our method:
the test function class $\TestFunctionClass{}$, the policy class
$\PolicyClass$, and the $Q$-function class $\Qclass{}$.  In this
section, we state a general guarantee (\cref{thm:NewPolicyEvaluation})
that involves the metric entropies of these sets.  In
Section~\ref{SecCorollaries}, we provide corollaries of this guarantee
for specific function classes.


In more detail, we equip the test function class and the $Q$-function
class with the usual sup-norm
\begin{align*}
\|f - \ftil\|_\infty \defeq \sup_{\psai} |f\psai - \ftil \psai|, \quad
\mbox{and} \quad \|Q - \Qtil\|_\infty \defeq \sup_{\psa} |Q \psa -
\Qtil \psa|,
\end{align*}
and the policy class with the sup-TV norm
\begin{align*}
  \|\pi - \pitil\|_{\infty, 1} & \defeq \sup_{\state} \|\pi(\cdot \mid
  \state) - \pitil(\cdot \mid \state) \|_1 = \sup_{\state}
  \sum_{\action} |\pi(\action \mid \state) - \pitil(\action \mid
  \state)|.
\end{align*}
For a given $\precision > 0$, we let
$\CoveringNumber{\TestFunctionClass{}}{\precision}$,
$\CoveringNumber{\Qclass{}}{\precision}$, and
$\CoveringNumber{\PolicyClass}{\precision}$ denote the
$\precision$-covering numbers of each of these function classes in the
given norms.  Given these covering numbers, a tolerance parameter
$\delta \in (0,1)$ and the shorthand $\Mfun(t) = \max \{t, \sqrt{t} \}$, define the radius function
\begin{subequations}
\label{EqnTheoremChoice}
\begin{align}
\label{EqnDefnR}
\Rad(\epsilon, \delta) & \defeq \nSamples \Big\{
\int_{\epsilon^2}^\epsilon \Mfun \big( \frac{\log
  N_u(\TestFunctionClass{})}{\numobs} \big) du + \frac{\log
  N_\epsilon(\Qclass{})}{\numobs} + \frac{ \log
  N_\epsilon(\Pi)}{\numobs} + \frac{\log(\numobs/\delta)}{\numobs}
\Big\}.
\end{align}
In our theorem, we implement the estimator using a radius $\Rad =
\Rad(\epsilon, \delta)$, where $\epsilon > 0$ is any parameter that
satisfies the bound
\begin{align}
\label{EqnRadChoice}
\epsilon^2 & \stackrel{(i)}{\leq} \cspec \: \frac{\Rad(\epsilon,
  \delta)}{\numobs}, \quad \mbox{and} \quad \regpar \stackrel{(i)}{=}
4 \frac{\Rad(\epsilon, \delta)}{\numobs}.
\end{align}
\end{subequations}
Here $\cspec > 0$ is a suitably chosen but universal constant (whose
value is determined in the proof), and we adopt the shorthand $\Rad =
\Rad(\epsilon, \delta)$ in our statement below.

\renewcommand{\descriptionlabel}[1]{%
  \hspace{\labelsep}\normalfont\underline{#1}% 
}

\begin{theorem}[High-probability guarantees]
\label{thm:NewPolicyEvaluation}
Consider the estimates implemented using triple $\InputFunctionClass$
that is weakly Bellman realizable (\cref{asm:WeakRealizability}); an
adapted dataset (\Cref{asm:Dataset}); and with the
choices~\eqref{EqnTheoremChoice} for $(\epsilon, \Rad, \regpar)$.
Then with probability at least $1 - \delta$:
\vspace{0.05in}
\begin{description}
\item[Policy evaluation:] For any $\pi \in \PolicyClass$, the
  estimates $(\VminEmp{\policy}, \VmaxEmp{\policy})$ specify a
  confidence interval satisfying the coverage~\eqref{EqnCoverage} and
  width bounds~\eqref{EqnWidthBound}.
  %
\item[Policy optimization:] Any max-min
  policy~\eqref{eqn:MaxMinEmpirical} $\piemp$ satisfies the oracle
  inequality~\eqref{EqnOracle}.
\end{description}
\end{theorem}
\noindent See \cref{SecProofNewPolicyEvaluation} for the proof of the
claim. \\

\paragraph{Choices of $(\Rad, \epsilon, \regpar)$:}  Let us provide
a few comments about the choices of $(\Rad, \epsilon, \regpar)$ from
equations~\eqref{EqnDefnR} and~\eqref{EqnRadChoice}.  The quality of
our bounds depends on the size of the constraint set
$\PopulationFeasibleSet{\policy}$, which is controlled by the
constraint level $\sqrt{\frac{\Rad}{\numobs}}$.  Consequently, our
results are tightest when $\Rad = \Rad(\epsilon, \delta)$ is as small
as possible.  Note that $\Rad$ is an decreasing function of
$\epsilon$, so that in order to minimize it, we would like to choose
$\epsilon$ as large as possible subject to the
constraint~\eqref{EqnRadChoice}(i).  Ignoring the entropy integral
term in equation~\eqref{EqnRadChoice} for the moment---see below for
some comments on it---these considerations lead to
\begin{align}
\numobs \epsilon^2 \asymp \log N_\epsilon(\TestFunctionClass{}) + \log
N_\epsilon(\Qclass{}) + \log N_\epsilon(\Pi).
\end{align}
This type of relation for the choice of $\epsilon$ in non-parametric
statistics is well-known (e.g., see Chapters 13--15 in the
book~\cite{wainwright2019high} and references therein).  Moreover,
setting $\regpar \asymp \epsilon^2$ as in
equation~\eqref{EqnRadChoice}(ii) is often the correct scale of
regularization.

\paragraph{Key technical steps in proof:}   It is worthwhile
making a few comments about the structure of the proof so as to
clarify the connections to \Cref{prop:Deterministic} along with the
weak formulation that underlies our methods.  Recall that
\Cref{prop:Deterministic} requires the empirical
$\EmpiricalFeasibleSet{\policy}$ and population sets
$\PopulationFeasibleSet{\policy}$ to satisfy the sandwich
relation~\eqref{EqnSandwich}.  In order to prove that this condition
holds with high probability, we need to establish uniform control over
the family of random variables
\begin{align}
\label{EqnKeyFamily}  
  \frac{ \big| \inprod{f}{\delta^\policy(\Qfnc)}_\numobs -
    \inprod{f}{\BellError^\policy(\Qfnc)}_\mudist
    \big|}{\TestNormaRegularizerEmp{}}, \qquad \mbox{as indexed by the
    triple $(f, \Qfnc, \policy)$.}
\end{align}
Note that the differences in the numerator of these variables
correspond to moving from the empirical constraints on $Q$-functions
that are enforced using the TD errors, to the population constraints
that involve the Bellman error function.

Uniform control of the family~\eqref{EqnKeyFamily}, along with the
differences $\|f\|_\numobs - \|f\|_\mudist$ uniformly over $f$, allows
us to relate the empirical and population sets, since the associated
constraints are obtained by shifting between the empirical inner
products $\inprod{\cdot}{\cdot}_\numobs$ to the reference inner
products $\inprod{\cdot}{\cdot}_\mudist$.  A simple discretization
argument allows us to control the differences uniformly in $(\Qfnc,
\policy)$, as reflected by the metric entropies appearing in our
definition~\eqref{EqnTheoremChoice}.  Deriving uniform bounds over
test functions $f$---due to the self-normalizing nature of the
constraints---requires a more delicate argument.  More precisely, in
order to obtain optimal results for non-parametric problems (see
Corollary~\ref{cor:alpha} to follow), we need to localize the
empirical process at a scale $\epsilon$, and derive bounds on the
localized increments.  This portion of the argument leads to the
entropy integral---which is localized to the interval $[\epsilon^2,
  \epsilon]$---in our definition~\eqref{EqnDefnR} of the radius
function.

\paragraph{Intuition from the on-policy setting:}

In order to gain intuition for the statistical meaning of the
guarantees in~\cref{thm:NewPolicyEvaluation}, it is worthwhile
understanding the implications in a rather special case---namely, the
simpler on-policy setting, where the discounted occupation measure
induced by the target policy $\policy$ coincides with the dataset
distribution $\DatasetDistributionStateActions$.  Let us consider the
case in which the identity function $\1$ belongs to the test class
$\TestFunctionClass{\policy}$.  Under these conditions, for any $\Qfnc
\in \PopulationFeasibleSet{\policy}$, we can write
\begin{align*}
\max_{\Qfnc \in \PopulationFeasibleSet{\policy}} |\PolComplex| &
\stackrel{(i)}{=} \max_{\Qfnc \in \PopulationFeasibleSet{\policy}}|
\Expecti{\BellmanError{\Qfnc}{\policy}{}}{\mudist}|
\; \stackrel{(ii)}{\leq} \sqrt{1 + \regpar} \;
\sqrt{\frac{\Rad}{\numobs}},
\end{align*}
where equality (i) follows from the on-policy assumption, and step
(ii) follows from the definition of the set
$\PopulationFeasibleSet{\policy}$, along with the condition that $\1
\in \TestFunctionClass{\policy}$.  Consequently, in the on-policy
setting, the width bound~\eqref{EqnWidthBound} ensures that
\begin{align}
\label{EqnOnPolicy}
\abs{\VminEmp{\policy} - \VmaxEmp{\policy}} \leq 2 \frac{\sqrt{1 +
    \regpar}}{1-\discount} \sqrt{\frac{ \Rad}{\numobs}}.
\end{align}
In this simple case, we see that the confidence interval scales as
$\sqrt{\Rad/\numobs}$, where the quantity $\Rad$ is related to the
metric entropy via equation~\eqref{EqnRadChoice}.  In the more general
off-policy setting, the bound involves this term, along with
additional terms that reflect the cost of off-policy data.  We discuss
these issues in more detail in \cref{sec:Applications}.  Before doing
so, however, it is useful derive some specific corollaries that show
the form of $\Rad$ under particular assumptions on the underlying
function classes, which we now do.

\subsubsection{Some corollaries}
\label{SecCorollaries}

Theorem~\ref{thm:NewPolicyEvaluation} applies generally to triples of
function classes $\InputFunctionalSpace$, and the statistical error
$\sqrt{\frac{\Rad(\epsilon, \delta)}{\numobs}}$ depends on the metric
entropies of these function classes via the
definition~\eqref{EqnDefnR} of $\Rad(\epsilon, \delta)$, and the
choices~\eqref{EqnRadChoice}.  As shown in this section, if we make
particular assumptions about the metric entropies, then we can derive
more concrete guarantees.

\paragraph{Parametric and finite VC classes:}  One form of metric
entropy, typical for a relatively simple function class $\Gclass$
(such as those with finite VC dimension) scales as
\begin{align}
  \label{EqnPolyMetric}
  \log N_\epsilon(\Gclass) & \asymp d \; \log \big(\tfrac{1}{\epsilon}
  \big),
\end{align}
for some dimensionality parameter $d$.  For instance, bounds of this
type hold for linear function classes with $d$ parameters, and for
finite VC classes (with $d$ proportional to the VC dimension); see
Chapter 5 of the book~\cite{wainwright2019high} for more details.

\begin{corollary}
\label{cor:poly}  
Suppose each class of the triple $\InputFunctionClass$ has metric
entropy that is at most polynomial~\eqref{EqnPolyMetric} of order $d$.
Then for a sample size $\numobs \geq 2 d$, the claims of
Theorem~\ref{thm:NewPolicyEvaluation} hold with $\epsilon^2 =
d/\numobs$ and
\begin{align}
    \label{EqnPolyRchoice}
    \tilde{\Rad}\big( \sqrt{\tfrac{d}{\numobs}}, \delta \big) & \defeq
    c \; \Big \{ d \; \log \big( \frac{\numobs}{d} \big) + \log
    \big(\frac{\nSamples}{\delta} \big) \Big \},
  \end{align}
where $c$ is a universal constant.  
\end{corollary}
\begin{proof}
Our strategy is to upper bound the radius $\Rad$ from
equation~\eqref{EqnDefnR}, and then show that this upper bound
$\tilde{\Rad}$ satisfies the conditions~\eqref{EqnRadChoice} for the
specified choice of $\epsilon^2$.  We first control the term $\log
N_\epsilon(\TestFunctionClass{})$.  We have
\begin{align*}
\frac{1}{\sqrt{\numobs}} \int_{\epsilon^2}^\epsilon \sqrt{\log
  N_u(\TestFunctionClass{})} du & \leq \sqrt{\frac{d}{\numobs}} \;
\int_{0}^{\epsilon} \sqrt{\log(1/u)} du \; = \; \epsilon
\sqrt{\frac{d}{\numobs}} \; \int_0^1 \sqrt{\log(1/(\epsilon t))} dt \;
= \; c \epsilon \log(1/\epsilon) \sqrt{\frac{d}{\numobs}}.
\end{align*}
Similarly, we have
\begin{align*}
\frac{1}{\numobs} \int_{\epsilon^2}^\epsilon \log
N_u(\TestFunctionClass{}) du & \leq \epsilon \frac{d}{\numobs} \Big \{
\int_{\epsilon}^{1} \log(1/t) dt + \log(1/\epsilon) \Big \} \; \leq \;
c \, \epsilon \log(1/\epsilon) \frac{d}{\numobs}.
\end{align*}
Finally, for terms not involving entropy integrals, we have
\begin{align*}
  \max \Big \{ \frac{\log N_\epsilon(\Qclass{})}{\numobs}, \frac{\log
    N_\epsilon(\Pi)}{\numobs} \Big\} & \leq c \frac{d}{\numobs}
  \log(1/\epsilon).
\end{align*}
Setting $\epsilon^2 = d/\numobs$, we see that the required
conditions~\eqref{EqnRadChoice} hold with the specified
choice~\eqref{EqnPolyRchoice} of $\tilde{\Rad}$.
\end{proof}


\paragraph{Richer function classes:}
In the previous section, the metric entropy scaled logarithmically in
the inverse precision $1/\epsilon$.  For other (richer) function
classes, the metric entropy exhibits a polynomial scaling in the
inverse precision, with an exponent $\alpha > 0$ that controls the
complexity.  More precisely, we consider classes of the form
\begin{align}
  \label{EqnAlphaMetric}
  \log N_\epsilon(\Gclass) & \asymp \Big(\frac{1}{\epsilon}
  \Big)^\alpha.
\end{align}
For example, the class of Lipschitz functions in dimension $d$ has
this type of metric entropy with $\alpha = d$.  More generally, for
Sobolev spaces of functions that have $s$ derivatives (and the
$s^{th}$-derivative is Lipschitz), we encounter metric entropies of
this type with $\alpha = d/s$.  See Chapter 5 of the
book~\cite{wainwright2019high} for further background.

\begin{corollary}
\label{cor:alpha}  
Suppose that each function class $\InputFunctionClass$ has metric
entropy with at most \mbox{$\alpha$-scaling~\eqref{EqnAlphaMetric}}
for some $\alpha \in (0,2)$.  Then the claims of
Theorem~\ref{thm:NewPolicyEvaluation} hold with $\epsilon^2 =
(1/\numobs)^{\frac{2}{2 + \alpha}}$, and
  \begin{align}
 \label{EqnAlphaRchoice}
    \tilde{\Rad}\big((1/\numobs)^{\frac{1}{2 + \alpha}}, \delta \big)
    & = c \; \Big \{ \numobs^{\frac{\alpha}{2 + \alpha}} +
    \log(\nSamples/\delta) \Big \}.
  \end{align}
where $c$ is a universal constant.  
\end{corollary}
\noindent 
We note that for standard regression problems over classes with
$\alpha$-metric entropy, the rate $(1/\numobs)^{\frac{2}{2 + \alpha}}$
is well-known to be minimax optimal (e.g., see Chapter 15 in the
book~\cite{wainwright2019high}, as well as references therein).

\begin{proof}
  We start by controlling the terms involving entropy integrals.
In particular, we have
  \begin{align*}
\frac{1}{\sqrt{\numobs}} \int_{\epsilon^2}^\epsilon \sqrt{\log
  N_u(\TestFunctionClass{})} du & \leq \frac{c}{\sqrt{\numobs}} u^{1 -
  \tfrac{\alpha}{2}} \Big |_{0}^\epsilon \; = \;
\frac{c}{\sqrt{\numobs}} \epsilon^{1 - \tfrac{\alpha}{2}}.
  \end{align*}
Requiring that this term is of order $\epsilon^2$ amounts to enforcing
that $\epsilon^{1 + \frac{\alpha}{2}} \asymp (1/\sqrt{\numobs})$, or
equivalently that $\epsilon^2 \asymp (1/\numobs)^{\frac{2}{2 +
    \alpha}}$.

If $\alpha \in (0,1]$, then the second entropy integral converges and
is of lower order. Otherwise, if $\alpha \in (1,2)$, then we have
\begin{align*}    
\frac{1}{\numobs} \int_{\epsilon^2}^\epsilon \log
N_u(\TestFunctionClass{}) du & \leq \frac{c}{\numobs}
\int_{\epsilon^2}^\epsilon (1/u)^{\alpha} du \leq \frac{c}{\numobs}
(\epsilon^2)^{1 - \alpha}.
\end{align*}
Hence the requirement that this term is bounded by $\epsilon^2$ is
equivalent to $\epsilon^{2 \alpha} \succsim (1/\numobs)$, or
$\epsilon^2 \succsim (1/\numobs)^{1/\alpha}$.  When $\alpha \in
(1,2)$, we have $\frac{1}{\alpha} > \frac{2}{2 + \alpha}$, so that
this condition is milder than our first condition.

Finally, we have $ \max \big \{ \frac{\log
  N_\epsilon(\Qclass{})}{\numobs}, \frac{\log
  N_\epsilon(\Pi)}{\numobs} \big\} \leq \frac{c}{\numobs}
\big(1/\epsilon)^{\alpha}$, and requiring that this term scales as
$\epsilon^2$ amounts to requiring that $\epsilon^{2 +\alpha} \asymp
(1/\numobs)$, or equivalently $\epsilon^2 \asymp
(1/\numobs)^{\frac{2}{2 + \alpha}}$, as before.
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




